T-RECS: A Simulation Tool to Study the Societal Impact of Recommender Systems

Simulation has emerged as a popular method to study the long-term societal consequences of recommender systems. This approach allows researchers to specify their theoretical model explicitly and observe the evolution of system-level outcomes over time. However, performing simulation-based studies often requires researchers to build their own simulation environments from the ground up, which creates a high barrier to entry, introduces room for implementation error, and makes it difficult to disentangle whether observed outcomes are due to the model or the implementation. We introduce T-RECS, an open-sourced Python package designed for researchers to simulate recommendation systems and other types of sociotechnical systems in which an algorithm mediates the interactions between multiple stakeholders, such as users and content creators. To demonstrate the flexibility of T-RECS, we perform a replication of two prior simulation-based research on sociotechnical systems. We additionally show how T-RECS can be used to generate novel insights with minimal overhead. Our tool promotes reproducibility in this area of research, provides a unified language for simulating sociotechnical systems, and removes the friction of implementing simulations from scratch.

==> sections/discussion.tex <==
Our goal in developing TRECS was to provide a unified and flexible framework for conducting agent-based simulations of algorithmic systems. To ensure that our framework could allow for the realization of multiple research designs related to the effects of algorithmic systems, we replicated two agent-based simulation studies with very different scientific questions and simulation designs. By replicating findings from both \cite{chaney2018} as well as \cite{goel2016structural}, we demonstrate that the core components of TRECS can be leveraged to address a variety of scientific problems relevant to algorithmic systems. From a broader perspective, the numerous challenges our team encountered in replicating \cite{chaney2018} and \cite{goel2016structural} demonstrate that even well-conceptualized, influential simulation research is not necessarily easy to reproduce. Often, small changes in our implementation resulted in large changes in either the outcome metrics or the computational performance of our simulations, raising questions about the sensitivity and robustness of simulation findings as well as the computational prerequisites to conduct such studies in the first place.  

Our two replication studies demonstrate that the TRECS framework can enable reproducible, open-source agent-based simulation for a single study. Our content creators case study demonstrates another benefit of our platform across studies; studies conducted using the same simulation designs and toolkits can be more readily compared than studies addressing similar questions with different tools and designs. Our content creators case study leveraged the same simulation design as \cite{chaney2018}; therefore, the homogenizing effects of algorithmic confounding on content creators can be wholly attributed to the addition of content creators rather than to any other differences in the simulation design or implementation. Moving forward, researchers who use TRECS to conduct simulation studies can likewise take our replication study code and extend our findings in new ways to answer novel scientific questions and can contribute to future extensions of their results by open-sourcing their own TRECS simulation code. 

Both the within and between study benefits of TRECS that we demonstrated through our case studies illustrate two broader problems with current research using agent-based simulations to understand algorithmic systems. At present, research in this domain is lacking both in transparency and in standardization. The absence of either transparency or standardization alone is not necessarily a problem. Early in a discipline’s development, researchers will address scientific questions using heterogeneous operationalization of theoretical constructs and with heterogeneous methods. This heterogeneity can lead to genuine scientific insight as researchers identify new and better ways to answer similar questions, but only when the sources of heterogeneity are readily identifiable. That is, heterogeneity of approaches or method without transparency cannot facilitate meaningful scientific debate; it can only contribute noise. Within the domain of agent-based simulation of algorithmic systems, researchers have not yet converged on any standardized approaches or methods, and public sharing of source code is not the standard. If source code were publicly available for all simulations, other researchers could pinpoint the origin of any differences between prior simulation studies and their own research, albeit painstakingly. Likewise, if the methods and tools for agent-based simulations were more standardized, differences in results could be more readily attributed to differences in conceptual or operational definitions or to underlying assumptions, even if no source code existed. 

TRECS contributes both to standardization of methods as well as transparency, at least for researchers who choose to share the source code of simulations they conduct using our platform. Yet as the field matures, convergence on other tools, methods, and processes will be necessary. This is not to say that any single method, theory, or approach is sufficient to address all questions relevant to the societal effects of algorithmic systems. Instead, we argue only that ambiguities in conceptual or operational constructs should be clarified and that where differences in approaches or variable conceptualizations exist, how they have been realized within a simulation should be readily identifiable through methodology write ups, source code, and code documentation. 





%Second, we want T-RECS to be the \texttt{scikit-learn} of algorithmic system simulation, democratizing simulation much like the popular package \texttt{scikit-learn} did with machine learning. To this end, \textit{can we develop a standard language to describe common simulation settings? Can we facilitate reproducibility by providing a unified simulation tool? Can we find shared principles across seemingly distinct problems?} Comparing previous studies is hard because they are often based on one-off simulators with different requirements. Furthermore, the multidisciplinary interest in this area complicates the terminology used to describe these requirements. T-RECS can contribute to the standardization of the language in the literature and the promotion of reproducibility because it is easy to use for simple experiments and fully configurable for complex studies.
\subsection{Future work}

There are several directions we aim to explore with T-RECS. 

First, we aim to validate and expand on the simulation and empirical literature with a large-scale replication study. For example, \textit{do findings generalize in realistic social networks with millions of users? Can we contextualize widely-cited studies yielding contradicting results on the existence of filter bubbles (e.g., \cite{moller2018not, geschke2019triple})?} Replicating prior work is typically hard, partly because reproducing the experiments is challenging and time-consuming.% T-RECS is well-suited for this problem as it is designed to minimize the engineering efforts required to develop a simulator.


\awnote{again, I am not sure the content below is necessary to motivate the current goals of this work. It may serve better in a discussion to address some sort of objection that there is no point to creating a unified framework for simulation that is based on relatively simple components. For example, you could have some discussion part that says something like "One potential objection to providing a unified framework with relatively simple system components is that real-world systems involve many components with complex structures and behaviors. However, we contend that critical scientific insights are frequently derived from simplified methodologies..blah blah blah..Schelling study is simple but powerful. Furthermore, the enterprise of experimental laboratory research, which is often considered the gold-standard method for empirical discovery, typically involves highly controlled and therefore highly ecologically invalid set ups. Yet the degree of experimental control enabled by synthetic laboratory set ups allow researchers to investigate specific causal mechanisms that are difficult to isolate in noisy real-world environments. Furthermore, although the default set up of T-RECS is simple to allow for better generalizability, T-RECS components are flexible enough to allow for arbitrarily complex specifications. As a result, researchers are able to calibrate the complexity or inherent noise in component behavior in a way that best suits their research goals.}
On the other hand, validating simulation models against real-world systems is challenging. This can be an argument in favor of complex models that closely resemble real-world recommender systems, which can be run by researchers to study counterfactuals and by engineers to test the effects of specific design choices. In the absence of details about the design of a system, as is often the case, models can be approximated by observing the outputs of real-world systems.

We argue that there is value in studying toy problems to generate intuition and discover core principles of the dynamics of recommender systems. Scientific disciplines such as physics often use simple models to isolate relevant aspects of a problem and make it easily understandable \cite{reutlinger2018understanding}. Free body diagrams in mechanics are an instance of such a conceptual simplification. An example closer to computational simulation is Schelling's enormously popular model of racial segregation \cite{schelling1971dynamic}. With the impact of recommender systems still largely unknown, there is still demand for methods that can shed light on fundamental characteristics caused by the long-term evolution of these systems. Simulation is a suitable analysis tool for recommender systems because of its focus on dynamics.
